Full likelihood inference for max-stable data

We show how to perform full likelihood inference for max-stable multivariate distributions or processes based on a stochastic Expectation-Maximisation algorithm, which combines statistical and computational efficiency in high-dimensions. The good performance of this methodology is demonstrated by simulation based on the popular logistic and Brown--Resnick models, and it is shown to provide dramatic computational time improvements with respect to a direct computation of the likelihood. Strategies to further reduce the computational burden are also discussed.

==> teachingmacros.tex <==
% LaTeX macros

% Last modified: 25/12/08

%----------------------------------------------
%  Anthony Davison, Department of Mathematics,
%  EPFL, 1015 Lausanne, Switzerland
%  00 41 21 693 5502
%  Anthony.Davison@epfl.ch
%----------------------------------------------

% teaching macros

\def\redbf#1{{\color{red}\bf #1}}%
\def\red#1{{\color{red} #1}}%
\def\b#1{{\color{red}\bf #1}}%
\def\Defn{\redbf{Definition:\ }}%
\def\Thm#1{\redbf{Theorem #1:\ }}%
\def\Ex#1{\redbf{Example #1:\ }}%
\def\Note{\redbf{Note:\ }}%
\def\Exercise#1{\redbf{Exercise #1:\ }}%
\def\Ill{\redbf{Illustration:\ }}%
\def\endex{{\hfill\redbf{$\bullet$}\smallskip}}
\def\eme{{\`eme}}
\def\ere{{\`ere}}

\def\picbox#1#2#3{{\centerline{\psfig{figure=#1,height=#2pc,angle=#3}}}}%

\def\tt#1{{\texttt{#1}}}
\def\Der#1{\textbf{D#1}}

\newtheorem{defn}{Definition}
\newtheorem{alg}[defn]{Algorithm}
\newtheorem{theorem}[defn]{Theorem}
\newtheorem{lemma}[defn]{Lemma}
\newtheorem{example}[defn]{Example}
\newtheorem{cor}[defn]{Corollary}
\newtheorem{prop}[defn]{Proposition}

\def\ssim{{\ {\buildrel s\over \sim}\ }}
\def\vsim{{\ {\buildrel v\over \sim}\ }}

\def\halfback{{\vspace{-0.1in}}}
\def\back{{\vspace{-0.2in}}}
